In a Nutshell, the Human Asked for This: Latent Goals for Following Temporal Specifications

We address the problem of building agents whose goal is to learn to execute out-of distribution (OOD) multi-task instructions expressed in temporal logic (TL) by using deep reinforcement learning (DRL). Recent works provided evidence that the agent's neural architecture is a key feature when DRL agents are learning to solve OOD tasks in TL. Yet, the studies on this topic are still in their infancy. In this work, we propose a new deep learning configuration with inductive biases that lead agents to generate latent representations of their current goal, yielding a stronger generalization performance. We use these latent-goal networks within a neuro-symbolic framework that executes multi-task formally-defined instructions and contrast the performance of the proposed neural networks against employing different state-of-the-art (SOTA) architectures when generalizing to unseen instructions in OOD environments.

==> utils/Archs_old.tex <==
\begin{figure}[t] 
\centering
% \hfill
    \begin{subfigure}{0.42\textwidth}
     \begin{adjustbox}{width=\linewidth} % rescale box
        \begin{tikzpicture}
                [
        base/.style = {rectangle, rounded corners, draw=black,
                                       minimum width=1cm, minimum height=1cm,
                                       text centered, font=\sffamily},
            Map/.style = {rectangle, draw=black, fill=brown!10, minimum width=1.2cm, minimum height=1cm},
            Spec/.style = {rectangle, draw=black, fill=red!30, minimum width=1.2cm, minimum height=0.3cm},
            FullyC/.style = {base, fill=re!15},
            Conv/.style = {base, fill=blue!15},
            CM/.style = {base, fill=orange!15},
            LSTM/.style = {base, fill=green!15},
            MAX/.style = {base, fill=pink!15},
            activation/.style = {base, minimum width=0.8 cm, minimum height=0.3cm, fill=orange!15,
                                       font=\ttfamily},
            output/.style = {base, minimum width=0.5cm, minimum height=0.5cm, fill=white,
                                       font=\ttfamily},
            node distance=1.4cm,
            every node/.style={fill=white, font=\sffamily}, align=center
            ]
            % Specification of nodes
            \node (MapI) [Map]   {\scriptsize Obs};
            \node (SpecE) [Spec, node distance=0.7cm, above of=MapI]   {\scriptsize Task};
            \node (Enc) [Conv, above right=-0.8cm and 0.6cm of MapI] {\scriptsize Encoder};
            % [below left=1cm and 3cm of a]
            \node (CM1) [CM, right of=Enc]  {\scriptsize Central\\ \scriptsize module};
            \node (action) [node distance=1.25cm, above right of= CM1]  {\scriptsize $a_{t-1}$};
            \node (LSTM1) [LSTM, right of=CM1]  {\scriptsize LSTM};
            \node (Actor) [output, above right= -0.2cm and 0.2cm of LSTM1] {\scriptsize $\pi(a_t)$};
            \node (Critic) [output, below right= -0.2cm and 0.2cm of LSTM1] { \scriptsize $V_t$};
        % % \node (Relu1)     [activation, node distance=0.45cm, above of=ConvL1]  {\scriptsize ReLu};
        % \node (Max) [MAX, above of=ConvL1]  {\scriptsize Max 3x3, stride 2};
       
        %  \node (Res1) [Res, above of=Max]  {\scriptsize Residual Block};
        %   \node (Res2) [Res, above of=Res1]  {\scriptsize Residual Block};
        %   \node (Relu2) [activation, node distance=1cm, above of=Res2]  {\scriptsize ReLu};
        % \node (Dense1)     [FullyC, above of=Relu2]  {\scriptsize FC 128};
        % \node (Relu3)     [activation, node distance=0.45cm, above of=Dense1]  {\scriptsize ReLu};
        % \node (Actor) [output, node distance=1cm, above right of=Relu3] {\scriptsize $\pi(a)$};
        % \node (Critic) [output, node distance=1cm, above left of=Relu3] { \scriptsize $V_t$};
        
        %Lines between nodes
        
        % \draw[->] (MapI) -- (Enc);
        \draw[->] (Enc) -- (CM1);
        \draw[->] (CM1) -- (LSTM1);
        \draw[->] (action) -- (LSTM1);
        \draw[->] (LSTM1) -- (Actor);
        \draw[->] (LSTM1) -- (Critic);
        \draw[thick,dashed] (0.5,1.15) -- (0.8,1.15);
        \draw[thick,dashed] (0.5,-0.7) -- (0.8,-0.7);
        \draw[thick,dashed] (0.8,-0.7) -- (0.8,1.15);
        \draw[->] (0.8,0.2) -- (Enc);
        % \draw[thick,dashed] (0.5,4.8) -- (1.5,4.8);
        % \draw[thick,dashed] (1.5,1.15) -- (1.5,4.8);
        %"Caption"
        %  \node [below of= MapI]
        %     {
        %         \scriptsize ResNet
        %     };
        % \node [right of= Res1, node distance=2cm]
        %     {
        %         \scriptsize x3\\
        %         \scriptsize [64,64,32] ch.
        %     };
        \end{tikzpicture}
    \end{adjustbox}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.54\textwidth}
    \begin{adjustbox}{width=\linewidth} % rescale box
            \begin{tikzpicture}
                    [
            base/.style = {rectangle, rounded corners, draw=black,
                                           minimum width=1cm, minimum height=1cm,
                                           text centered, font=\sffamily},
                Map/.style = {rectangle, draw=black, fill=brown!10, minimum width=1.2cm, minimum height=1cm},
                Spec/.style = {rectangle, draw=black, fill=red!30, minimum width=1.2cm, minimum height=0.3cm},
                FullyC/.style = {base, fill=blue!5},
                Conv/.style = {base, fill=blue!15},
                CM/.style = {base, fill=orange!15},
                LSTM/.style = {base, fill=green!15},
                MAX/.style = {base, fill=pink!15},
                activation/.style = {base, minimum width=0.8 cm, minimum height=0.3cm, fill=orange!15,
                                           font=\ttfamily},
                output/.style = {base, minimum width=0.5cm, minimum height=0.5cm, fill=white,
                                           font=\ttfamily},
                node distance=1.4cm,
                every node/.style={fill=white, font=\sffamily}, align=center
                ]
                % Specification of nodes
                \node (MapI) [Map]   {\scriptsize Obs};
                \node (Spec) [Spec, node distance=0.7cm, above of=MapI]   {\scriptsize Task};
                \node (Enc) [Conv, above right=-0.8cm and 0.5cm of MapI] {\scriptsize Encoder};
            
                \node (EncMap) [Map, fill=brown!30, below right=-0.4cm and 0.6cm of Enc]   {\scriptsize Encoded \\ \scriptsize Obs};
                \node (EncSpec) [Spec, node distance=1.2cm, above of=EncMap]   {\tiny Encoded \\ \tiny Task};
                % [below left=1cm and 3cm of a]
                \node (CM1) [CM, above right= -0.4cm and 0.6cm of EncMap]  {\scriptsize Central\\ \scriptsize module 1};
                \node (action1) [node distance=1.25cm, above right of= CM1]  {\scriptsize $a_{t-1}$};
                \node (LSTM1) [LSTM, right of=CM1]  {\scriptsize LSTM \\ \scriptsize 128};
                \node (FC) [FullyC, right of=LSTM1, minimum height=0.5cm]  {\tiny FC 16};
                \node (CM2) [CM, node distance=2.2cm, below of=EncMap]  {\scriptsize Central\\ \scriptsize module 2};
                
                \node (SUM) [output, right of=CM2]  { $+$};
                \node (action2) [above right= 0.4cm and -0.1cm of SUM]  {\scriptsize $a_{t-1}$};
                \node (LSTM2) [LSTM, right of=SUM]  {\scriptsize LSTM \\ \scriptsize 128};
                \node (Actor) [output, above right= -0.2cm and 0.2cm of LSTM2] {\scriptsize $\pi(a_t)$};
                \node (Critic) [output, below right= -0.2cm and 0.2cm of LSTM2] { \scriptsize $V_t$};
            % % \node (Relu1)     [activation, node distance=0.45cm, above of=ConvL1]  {\scriptsize ReLu};
            % \node (Max) [MAX, above of=ConvL1]  {\scriptsize Max 3x3, stride 2};
           
            %  \node (Res1) [Res, above of=Max]  {\scriptsize Residual Block};
            %   \node (Res2) [Res, above of=Res1]  {\scriptsize Residual Block};
            %   \node (Relu2) [activation, node distance=1cm, above of=Res2]  {\scriptsize ReLu};
            % \node (Dense1)     [FullyC, above of=Relu2]  {\scriptsize FC 128};
            % \node (Relu3)     [activation, node distance=0.45cm, above of=Dense1]  {\scriptsize ReLu};
            % \node (Actor) [output, node distance=1cm, above right of=Relu3] {\scriptsize $\pi(a)$};
            % \node (Critic) [output, node distance=1cm, above left of=Relu3] { \scriptsize $V_t$};
            
            %Lines between nodes
            
            % \draw[->] (MapI) -- (Enc);
            % \draw[->] (Enc) -- (CM1);
            \draw[->] (CM1) -- (LSTM1);
            \draw[->] (action1) -- (LSTM1);
            \draw[->] (action2) -- (LSTM2);
            \draw[->] (LSTM1) -- (FC);
            \draw[->] (CM2) -- (SUM);
            \draw[->] (SUM) -- (LSTM2);
            \draw[->] (LSTM2) -- (Actor);
            \draw[->] (LSTM2) -- (Critic);
            % First bracket
            \draw[thick,dashed] (0.4,1) -- (0.7,1);
            \draw[thick,dashed] (0.5,-0.6) -- (0.7,-0.6);
            \draw[thick,dashed] (0.7,-0.6) -- (0.7,1);
            \draw[->] (0.7,0.2) -- (Enc);
            % Encoder to output
            % \draw[->] (Enc) -- (2.7,0.2);
            \draw[->] (Enc) -- (EncSpec);
            \draw[->] (Enc) -- (EncMap);
            % Second bracket
            % \draw[thick,dashed] (3.9,1.3) -- (4.2,1.3);
            % \draw[thick,dashed] (3.9,-1) -- (4.2,-1);
            % \draw[thick,dashed] (4.2,-1) -- (4.2,1.3);
            % \draw[->] (4.2,0.2) -- (CM1)
            \draw[->] (EncSpec) -- (CM1);
            \draw[->] (EncMap) -- (CM1);
            
            % Navigator input
            % \draw[blue] (2.7,-1.1) rectangle (4.3,0.15);
            % \draw[blue] (3.5,-0.4) ellipse (0.9 and 0.7);
            % \draw[->] (3.485,-1.1) -- (CM2);
            \draw[->] (EncMap) -- (CM2);
            % Joining modules
            \draw[->] (FC) .. controls (8.2,-0.5) and  (3.3,-0.6).. (SUM);
            
            % Modules
            \draw[red,dashed] (4.5,-0.5) rectangle (8.7,1.5);
            \node at (7.9,1.1)
                {
                    \scriptsize \textcolor{red}{Translator}
                };
            \draw[red,dashed] (2.5,-3.9) rectangle (8.7,-1.4);
             \node at (3.4,-3.5)
                {
                    \scriptsize \textcolor{red}{Actuator}
                };
            
            % (-2,2) .. controls (-1,0) and (1,0) .. (2,2);
            
            % Navigator input
            % \draw[thick,dashed, color=red!60] (4.2,-0.8) -- (4.2,1.5);
            %"Caption"
            %  \node [below of= MapI]
            %     {
            %         \scriptsize ResNet
            %     };
            % \node [right of= Res1, node distance=2cm]
            %     {
            %         \scriptsize x3\\
            %         \scriptsize [64,64,32] ch.
            %     };
            \end{tikzpicture}
    \end{adjustbox}
    \end{subfigure}%%

\caption{ \textbf{Left:} standard neural network architecture. The encoder is a 3-layer CNN that receives observations with tasks as input. The central module can be either a fully connected layer (MLP), an RN, an MHA or a PrediNet. Outputs $\pi(a_t)$ and $V_t$ refer to the actor and critic respectively \cite{mnih2016asynchronous}. \textbf{Right:} architecture with inductive latent goals. Here the \textit{translator} modules generate a latent goal given the SATTL task and the observation, which is concatenated with the output of central module 2 (CM2) of the \textit{actuator}. CM2 has no information of the current task. CM1 and CM2 are always the same type of network except for the PNMHA\SP{LG} and MHAPN\SP{LG} in Sec.~\ref{sec:Ablation} where they differ. \bg{remove translator and actuator naming and add a pointer of latent goal and task-agonostic. Substitute LSTM by generic recurrent layer naming, put a square highlighting decision-making layers in each configuration, substitute FC 16 by Information bottleneck}}
\label{fig:Archs}
\end{figure}

==> utils/MMArch.tex <==
\begin{figure}[t] 
\centering
% \hfill
    \begin{adjustbox}{width=0.48\linewidth} % rescale box
        \begin{tikzpicture}
                [
        base/.style = {rectangle, rounded corners, draw=black,
                                       minimum width=1cm, minimum height=1cm,
                                       text centered, font=\sffamily},
            Map/.style = {rectangle, draw=black, fill=brown!10, minimum width=1.2cm, minimum height=1cm},
            Spec/.style = {rectangle, draw=black, fill=red!30, minimum width=1.2cm, minimum height=0.3cm},
            FullyC/.style = {base, fill=blue!5},
            Conv/.style = {base, fill=blue!15},
            CM/.style = {base, fill=orange!15},
            LSTM/.style = {base, fill=green!15},
            MAX/.style = {base, fill=pink!15},
            activation/.style = {base, minimum width=0.8 cm, minimum height=0.3cm, fill=orange!15,
                                       font=\ttfamily},
            output/.style = {base, minimum width=0.5cm, minimum height=0.5cm, fill=white,
                                       font=\ttfamily},
            node distance=1.4cm,
            every node/.style={fill=white, font=\sffamily}, align=center
            ]
            % Specification of nodes
            \node (MapI) [Map]   {\scriptsize Obs};
            \node (Spec) [Spec, node distance=0.7cm, above of=MapI]   {\scriptsize Task};
            \node (Enc) [Conv, above right=-0.8cm and 0.5cm of MapI] {\scriptsize Encoder};
        
            \node (EncMap) [Map, fill=brown!30, below right=-0.4cm and 0.6cm of Enc]   {\scriptsize Encoded \\ \scriptsize Obs};
            \node (EncSpec) [Spec, node distance=1.2cm, above of=EncMap]   {\tiny Encoded \\ \tiny Task};
            % [below left=1cm and 3cm of a]
            \node (CM1) [CM, above right= -0.4cm and 0.6cm of EncMap]  {\scriptsize Central\\ \scriptsize module 1};
            \node (action1) [node distance=1.25cm, above right of= CM1]  {\scriptsize $a_{t-1}$};
            \node (LSTM1) [LSTM, right of=CM1]  {\scriptsize LSTM \\ \scriptsize 128};
            \node (FC) [FullyC, right of=LSTM1, minimum height=0.5cm]  {\tiny FC 16};
            \node (CM2) [CM, node distance=2.2cm, below of=EncMap]  {\scriptsize Central\\ \scriptsize module 2};
            
            \node (SUM) [output, right of=CM2]  { $+$};
            \node (action2) [above right= 0.4cm and -0.1cm of SUM]  {\scriptsize $a_{t-1}$};
            \node (LSTM2) [LSTM, right of=SUM]  {\scriptsize LSTM \\ \scriptsize 128};
            \node (Actor) [output, above right= -0.2cm and 0.2cm of LSTM2] {\scriptsize $\pi(a)$};
            \node (Critic) [output, below right= -0.2cm and 0.2cm of LSTM2] { \scriptsize $V_t$};
        % % \node (Relu1)     [activation, node distance=0.45cm, above of=ConvL1]  {\scriptsize ReLu};
        % \node (Max) [MAX, above of=ConvL1]  {\scriptsize Max 3x3, stride 2};
       
        %  \node (Res1) [Res, above of=Max]  {\scriptsize Residual Block};
        %   \node (Res2) [Res, above of=Res1]  {\scriptsize Residual Block};
        %   \node (Relu2) [activation, node distance=1cm, above of=Res2]  {\scriptsize ReLu};
        % \node (Dense1)     [FullyC, above of=Relu2]  {\scriptsize FC 128};
        % \node (Relu3)     [activation, node distance=0.45cm, above of=Dense1]  {\scriptsize ReLu};
        % \node (Actor) [output, node distance=1cm, above right of=Relu3] {\scriptsize $\pi(a)$};
        % \node (Critic) [output, node distance=1cm, above left of=Relu3] { \scriptsize $V_t$};
        
        %Lines between nodes
        
        % \draw[->] (MapI) -- (Enc);
        % \draw[->] (Enc) -- (CM1);
        \draw[->] (CM1) -- (LSTM1);
        \draw[->] (action1) -- (LSTM1);
        \draw[->] (action2) -- (LSTM2);
        \draw[->] (LSTM1) -- (FC);
        \draw[->] (CM2) -- (SUM);
        \draw[->] (SUM) -- (LSTM2);
        \draw[->] (LSTM2) -- (Actor);
        \draw[->] (LSTM2) -- (Critic);
        % First bracket
        \draw[thick,dashed] (0.4,1) -- (0.7,1);
        \draw[thick,dashed] (0.5,-0.6) -- (0.7,-0.6);
        \draw[thick,dashed] (0.7,-0.6) -- (0.7,1);
        \draw[->] (0.7,0.2) -- (Enc);
        % Encoder to output
        % \draw[->] (Enc) -- (2.7,0.2);
        \draw[->] (Enc) -- (EncSpec);
        \draw[->] (Enc) -- (EncMap);
        % Second bracket
        % \draw[thick,dashed] (3.9,1.3) -- (4.2,1.3);
        % \draw[thick,dashed] (3.9,-1) -- (4.2,-1);
        % \draw[thick,dashed] (4.2,-1) -- (4.2,1.3);
        % \draw[->] (4.2,0.2) -- (CM1)
        \draw[->] (EncSpec) -- (CM1);
        \draw[->] (EncMap) -- (CM1);
        
        % Navigator input
        % \draw[blue] (2.7,-1.1) rectangle (4.3,0.15);
        % \draw[blue] (3.5,-0.4) ellipse (0.9 and 0.7);
        % \draw[->] (3.485,-1.1) -- (CM2);
        \draw[->] (EncMap) -- (CM2);
        % Joining modules
        \draw[->] (FC) .. controls (8.2,-0.5) and  (3.3,-0.6).. (SUM);
        
        % Modules
        \draw[red,dashed] (4.5,-0.5) rectangle (8.7,1.5);
        \node at (7.9,1.1)
            {
                \scriptsize \textcolor{red}{Translator}
            };
        \draw[red,dashed] (2.5,-3.9) rectangle (8.7,-1.4);
         \node at (3.4,-3.5)
            {
                \scriptsize \textcolor{red}{Actuator}
            };
        
        % (-2,2) .. controls (-1,0) and (1,0) .. (2,2);
        
        % Navigator input
        % \draw[thick,dashed, color=red!60] (4.2,-0.8) -- (4.2,1.5);
        %"Caption"
        %  \node [below of= MapI]
        %     {
        %         \scriptsize ResNet
        %     };
        % \node [right of= Res1, node distance=2cm]
        %     {
        %         \scriptsize x3\\
        %         \scriptsize [64,64,32] ch.
        %     };
        \end{tikzpicture}
    \end{adjustbox}       %

\caption{Multi-module architecture. Here the translator generates a latent goal representation given the SATTL task and the observation, which is concatenated with the output of central module 2 (CM2), that has no information of the given task. Again, the CMs can be either an MLP, RN, MHA or a PrediNet. CM1 and CM2 are always the same type of network except for the M-PNMHA and M-MHAPN in Sec.\ref{sec:Ablation} where they differ.}
\label{fig:MMArch}
\end{figure}

==> utils/stdArch.tex <==
\begin{figure}[t] 
\centering
% \hfill
    \begin{adjustbox}{width=0.5\linewidth} % rescale box
        \begin{tikzpicture}
                [
        base/.style = {rectangle, rounded corners, draw=black,
                                       minimum width=1cm, minimum height=1cm,
                                       text centered, font=\sffamily},
            Map/.style = {rectangle, draw=black, fill=brown!10, minimum width=1.2cm, minimum height=1cm},
            Spec/.style = {rectangle, draw=black, fill=red!30, minimum width=1.2cm, minimum height=0.3cm},
            FullyC/.style = {base, fill=re!15},
            Conv/.style = {base, fill=blue!15},
            CM/.style = {base, fill=orange!15},
            LSTM/.style = {base, fill=green!15},
            MAX/.style = {base, fill=pink!15},
            activation/.style = {base, minimum width=0.8 cm, minimum height=0.3cm, fill=orange!15,
                                       font=\ttfamily},
            output/.style = {base, minimum width=0.5cm, minimum height=0.5cm, fill=white,
                                       font=\ttfamily},
            node distance=1.4cm,
            every node/.style={fill=white, font=\sffamily}, align=center
            ]
            % Specification of nodes
            \node (MapI) [Map]   {\scriptsize Obs};
            \node (SpecE) [Spec, node distance=0.7cm, above of=MapI]   {\scriptsize Task};
            \node (Enc) [Conv, above right=-0.8cm and 0.6cm of MapI] {\scriptsize Encoder};
            % [below left=1cm and 3cm of a]
            \node (CM1) [CM, right of=Enc]  {\scriptsize Central\\ \scriptsize module};
            \node (action) [node distance=1.25cm, above right of= CM1]  {\scriptsize $a_{t-1}$};
            \node (LSTM1) [LSTM, right of=CM1]  {\scriptsize LSTM};
            \node (Actor) [output, above right= -0.2cm and 0.2cm of LSTM1] {\scriptsize $\pi(a)$};
            \node (Critic) [output, below right= -0.2cm and 0.2cm of LSTM1] { \scriptsize $V_t$};
        % % \node (Relu1)     [activation, node distance=0.45cm, above of=ConvL1]  {\scriptsize ReLu};
        % \node (Max) [MAX, above of=ConvL1]  {\scriptsize Max 3x3, stride 2};
       
        %  \node (Res1) [Res, above of=Max]  {\scriptsize Residual Block};
        %   \node (Res2) [Res, above of=Res1]  {\scriptsize Residual Block};
        %   \node (Relu2) [activation, node distance=1cm, above of=Res2]  {\scriptsize ReLu};
        % \node (Dense1)     [FullyC, above of=Relu2]  {\scriptsize FC 128};
        % \node (Relu3)     [activation, node distance=0.45cm, above of=Dense1]  {\scriptsize ReLu};
        % \node (Actor) [output, node distance=1cm, above right of=Relu3] {\scriptsize $\pi(a)$};
        % \node (Critic) [output, node distance=1cm, above left of=Relu3] { \scriptsize $V_t$};
        
        %Lines between nodes
        
        % \draw[->] (MapI) -- (Enc);
        \draw[->] (Enc) -- (CM1);
        \draw[->] (CM1) -- (LSTM1);
        \draw[->] (action) -- (LSTM1);
        \draw[->] (LSTM1) -- (Actor);
        \draw[->] (LSTM1) -- (Critic);
        \draw[thick,dashed] (0.5,1.15) -- (0.8,1.15);
        \draw[thick,dashed] (0.5,-0.7) -- (0.8,-0.7);
        \draw[thick,dashed] (0.8,-0.7) -- (0.8,1.15);
        \draw[->] (0.8,0.2) -- (Enc);
        % \draw[thick,dashed] (0.5,4.8) -- (1.5,4.8);
        % \draw[thick,dashed] (1.5,1.15) -- (1.5,4.8);
        %"Caption"
        %  \node [below of= MapI]
        %     {
        %         \scriptsize ResNet
        %     };
        % \node [right of= Res1, node distance=2cm]
        %     {
        %         \scriptsize x3\\
        %         \scriptsize [64,64,32] ch.
        %     };
        \end{tikzpicture}
    \end{adjustbox}       %
\caption{Standard neural network architecture. The encoder is a 3-layer CNN that receives extended observations as input. The central module can be either a fully connected layer (MLP), an RN, an MHA or a PrediNet.}
\label{fig:stdArch}
\end{figure}

==> utils/tables/table3_back_up.tex <==
\begin{table*}[t]
  \centering
  \normalsize
    \caption{Ablation study of PrediNet\SP{LG} (5 i.r. per variant). PrediNet\SPSB{LG}{noSub} and PrediNet\SPSB{LG}{noPos} are variants of PrediNet\SP{LG} that eliminate the element-wise subtraction and the feature coordinates respectively. PNMHA\SP{LG} uses an MHA in the CM2 of PrediNet\SP{LG}, while MHAPN\SP{LG} uses an MHA in CM1.\label{table:ablationPred}} 
    % \vskip 0.15in
  \mycfs{7.5}
  \begin{tabular}{ccccccccccc}
%   c{0.6cm}c{1.5cm}c{1.5cm}c{1.5cm}c{1.5cm}c{1.5cm}c{1.5cm}c{1.5cm}c{1.5cm}
    \toprule
 PrediNet & \multicolumn{2}{c}{  PrediNet\SPSB{LG}{noSub}} &  \multicolumn{2}{c}{PrediNet\SPSB{LG}{noPos}}  & \multicolumn{2}{c}{ PNMHA\SP{LG}} 
 & \multicolumn{2}{c}{MHAPN\SP{LG}}\\
\cmidrule(r){2-3}
\cmidrule(r){4-5}
\cmidrule(r){6-7}
\cmidrule(r){8-9}
 Map size & Train & Test & Train & Test & Train & Test &  Train & Test\\
% \midrule
  7x7  & 41$(8)$ &	22.8$(2.8)$ &	50.6$(9.9)$ & 29.3 $(5)$ & 39.3$(7.6)$ & 29.2$(6.2)$ & 49$(10)$ & 36.6$(7.5)$\\
  
 14x14  &64.7$(7.9)$
	& 42.3$(6.9)$ & 68.2$(10.8)$& 48.1$(5.4)$ & 52.8$(3.9)$ &	46.5 $(7.9)$& 
	59.9$(9.8)$ & 45.6$(4.9)$\\
 22x22 & 63.7$(7.8)$	& 46.4$(8.1)$ & 70.6$(9.3)$	& 56.4$(9.2)$	& 64.6$(6.7)$&	45.2$(10)$ & 57.4$(6.4)$ & 51.6$(7.6)$\\
 \midrule
Bottleneck \\ size & \multicolumn{2}{c}{ 4} &  \multicolumn{2}{c}{16}  & \multicolumn{2}{c}{ 64} 
  & \multicolumn{2}{c}{256}\\
\cmidrule(r){2-3}
\cmidrule(r){4-5}
\cmidrule(r){6-7}
\cmidrule(r){8-9}
  & Train & Test & Train & Test & Train & Test &  Train & Test &  Train & Test\\
% \midrule
  7x7  & 41$(8)$ &	22.8$(2.8)$ &	50.6$(9.9)$ & 29.3 $(5)$ & 39.3$(7.6)$ & 29.2$(6.2)$ & 49$(10)$ & 36.6$(7.5)$\\
  
 14x14  &64.7$(7.9)$
	& 42.3$(6.9)$ & 68.2$(10.8)$& 48.1$(5.4)$ & 52.8$(3.9)$ &	46.5 $(7.9)$& 
	59.9$(9.8)$ & 45.6$(4.9)$\\
 22x22 & 63.7$(7.8)$	& 46.4$(8.1)$ & 70.6$(9.3)$	& 56.4$(9.2)$	& 64.6$(6.7)$&	45.2$(10)$ & 57.4$(6.4)$ & 51.6$(7.6)$\\
\bottomrule
  \end{tabular}
\end{table*}

% \begin{table*}[t]
%   \centering
%   \normalsize
%     \caption{Ablation study of the M-PrediNet with 5 i.r. per variant. M-PrediNet-NoDiff and M-PrediNet-NoPos are variants that eliminate the element-wise subtraction and the feature coordinates respectively. M-PNMHA uses a MHA in the CM2 of the M-PrediNet, while the M-MHAPN uses the MHA in CM1.} 
%     \vskip 0.15in
%     \label{table:ablationPred}
%   \small
%   \begin{tabular}{ccccccccc}
% %   c{0.6cm}c{1.5cm}c{1.5cm}c{1.5cm}c{1.5cm}c{1.5cm}c{1.5cm}c{1.5cm}c{1.5cm}
%     \toprule
%     Map size  & \multicolumn{2}{c}{M-PrediNet-NoDiff} &  \multicolumn{2}{c}{M-PrediNet-NoPos}  & \multicolumn{2}{c}{M-PNMHA} 
%   & \multicolumn{2}{c}{M-MHAPN}\\
% \cmidrule(r){2-3}
% \cmidrule(r){4-5}
% \cmidrule(r){6-7}
% \cmidrule(r){8-9}
%   & Train & Test & Train & Test & Train & Test &  Train & Test\\
% % \midrule
%   7x7  & 50.6$(8.4$ &	27.7$(2.3$ &	55$(5.8$ & 34.4 $(7.0$ & 46.5$(5.6$ & 28.6$(4$ & 57.2$(14.6$ & 40.8$(3$\\
  
%  14x14  &76.8$(7.2$
% 	& 50$(5.5$ & 86.2$(13$& 57.7$(5$ & 61.8$(3.2$ &	56.7 $(12.2$& 
% 	72$(12.7$ & 54.1$(3.7$\\
%  22x22 & 72.9$(4.7$	& 53.7$(10.1$ & 78.6$(7.9$	& 65.1$(11.1$	& 73.5$(1.2$&	51.4$(13.2$ & 63.6$(6$ & 56.3$(7.1$\\
% \bottomrule
%   \end{tabular}
% \end{table*}
